A Comprehensive Survey of Challenges and Opportunities of Few-Shot Learning Across Multiple Domains

In a world where new domains are constantly discovered and machine learning (ML) is applied to automate new tasks every day, challenges arise with the number of samples available to train ML models. While the traditional ML training relies heavily on data volume, finding a large dataset with a lot of usable samples is not always easy, and often the process takes time. For instance, when a new human transmissible disease such as COVID-19 breaks out and there is an immediate surge for rapid diagnosis, followed by rapid isolation of infected individuals from healthy ones to contain the spread, there is an immediate need to create tools/automation using machine learning models. At the early stage of an outbreak, it is not only difficult to obtain a lot of samples, but also difficult to understand the details about the disease, to process the data needed to train a traditional ML model. A solution for this can be a few-shot learning approach. This paper presents challenges and opportunities of few-shot approaches that vary across major domains, i.e., audio, image, text, and their combinations, with their strengths and weaknesses. This detailed understanding can help to adopt appropriate approaches applicable to different domains and applications.

==> discussion.tex <==
\section{Discussion}\label{discussion}

Due to ease of use over knowledge-based authentications, biometric authentications have recently become popular. 
Traditional biometrics rely on more stable features such as the face, fingerprint, and iris. Compared to traditional biometrics, soft biometrics utilize less stable features, such as gait, signature, and cardiovascular signals. Future researchers need to consider various contexts and factors that affect soft biometrics before using these biometrics. 
Despite the higher accuracy and stability of traditional biometric-based authentications, they suffer from some shortcomings, including the requirement for powerful sensors and computing resources, which is not always possible for tiny IoT devices. On the other hand, soft biometrics can be easily obtained continuously from tiny IoT devices with less powerful sensing and computing capabilities. Though this continuous data acquisition does not require any active user input, they suffer from the low granularity of samples. Therefore, to better utilize traditional and soft biometrics to make our life comfortable and secure our cyber-physical space, we first need a detailed understanding of different biometrics and their limitations with applications, which we present in this manuscript.  


With the integration of more sensors and the enhancement of computing capabilities in IoT devices, we are now in the era of multi-modal biometric authentications. The promise of multi-modal biometrics relies on various levels of data fusion techniques, including data-level, feature-level, score-level, rank-level, and decision-level fusion~\cite{vhaduri2017towards,vhaduri2017wearable,vhaduri2018biometric,vhaduri2019multi}. In multi-modal approaches, data fusion from multiple biometrics will complement each other when authenticating an individual compared to the single biometric-based methods~\cite{dibbo2021onphone}. With the rise of IoT connectivity, it will be also promising to integrate biometrics from multiple IoT-connected devices of a user to better identify a user~\cite{cheung2020continuous,cheung2020context,muratyan2021opportunistic,vhaduri2021HIAuth}. 


In spite of its popularity, biometrics authentications are still relatively new to other security approaches, and with the integration of multiple devices new challenges and opportunities are being created every now and then. Therefore, more research is needed to secure the magnitude of devices connected to the internet. It will be important to investigate how to secure a wide range of areas, including health monitoring with tiny smartwatches. 
Also, in the future, we need to investigate how to better use these biometrics when deployed in other areas/activity, including criminal tracking in the surveillance system, student attendance tracking and evaluation in the education system, and contactless payments in the point-of-sale systems. 
A secure and comfortable future relies on the successful integration of biometrics. For example, continuous soft biometric data, such as heart rate and gait (obtained from smartwatches), can be integrated with traditional one-time fingerprint biometrics (received from smartphones) to lock/unlock smart homes/cars, or bank accounts. 
Another interesting direction will be to investigate how to combine multiple biometrics considering their availability due to device/sensor malfunctioning, data missing, and other issues. 
